The Writing is on the Wall: Analyzing the Boom of Inscriptions and its Impact on Rollup Performance and Cost Efficiency

Late 2023 witnessed significant user activity on EVM chains, resulting in a surge in transaction activity and putting many rollups into the first live test. While some rollups performed well, some others experienced downtime during this period, affecting transaction finality time and gas fees. To address the lack of empirical research on rollups, we perform the first study during a heightened activity during the late 2023 transaction boom, as attributed to inscriptions - a novel technique that enables NFT and ERC-20 token creation on Bitcoin and other blockchains. We observe that minting inscription-based meme tokens on zkSync Era allows for trading at a fraction of the costs, compared to the Bitcoin or Ethereum networks. We also found that the increased transaction activity, over 99% attributed to the minting of new inscription tokens, positively affected other users of zkSync Era, resulting in lowered gas fees. Unlike L1 blockchains, ZK rollups may experience lower gas fees with increased transaction volume. Lastly, the introduction of blobs - a form of temporary data storage - decreased the gas costs of Ethereum rollups, but also raised a number of questions about the security of inscription-based tokens.

==> Makefile <==
MAIN=main
SRCS=sections/*.tex

LMK=latexmk
OTYPE=-pdf
TEX=-pdflatex
TEX_OPTS="pdflatex -interaction=nonstopmode -shell-escape"
BIB=-bibtex

ERROR_MSG=Error: cannot find '$(LMK)' in path; try 'pdflatex $(MAIN).tex'

lmk_check =								\
	@which $(LMK) > /dev/null ||		\
		(echo "$(ERROR_MSG)" >& 2 &&	\
			exit 1)

default: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex $(SRCS)
	$(call lmk_check)
	@$(LMK) $(OTYPE) $(TEX)=$(TEX_OPTS) $(BIB) $<

.PHONY: watch clean

# Automatically rebuild latex files whenever changes are made.
watch: $(MAIN).tex
	$(call lmk_check)
	@$(LMK) -pvc $(OTYPE) $(TEX)=$(TEX_OPTS) $(BIB) $<

clean:
	@rm -f *.dvi *.aux *.blg *.log *.ps *~ *.bbl *.fdb_latexmk *.fls $(MAIN).pdf *.out

